LADDER: Multi-objective Backdoor Attack via Evolutionary Algorithm

Current black-box backdoor attacks in convolutional neural networks formulate attack objective(s) as single-objective optimization problems in single domain. Designing triggers in single domain harms semantics and trigger robustness as well as introduces visual and spectral anomaly. This work proposes a multi-objective black-box backdoor attack in dual domains via evolutionary algorithm (LADDER), the first instance of achieving multiple attack objectives simultaneously by optimizing triggers without requiring prior knowledge about victim model. In particular, we formulate LADDER as a multi-objective optimization problem (MOP) and solve it via multi-objective evolutionary algorithm (MOEA). MOEA maintains a population of triggers with trade-offs among attack objectives and uses non-dominated sort to drive triggers toward optimal solutions. We further apply preference-based selection to MOEA to exclude impractical triggers. We state that LADDER investigates a new dual-domain perspective for trigger stealthiness by minimizing the anomaly between clean and poisoned samples in the spectral domain. Lastly, the robustness against preprocessing operations is achieved by pushing triggers to low-frequency regions. Extensive experiments comprehensively showcase that LADDER achieves attack effectiveness of at least 99%, attack robustness with 90.23% (50.09% higher than state-of-the-art attacks on average), superior natural stealthiness (1.12x to 196.74x improvement) and excellent spectral stealthiness (8.45x enhancement) as compared to current stealthy attacks by the average $l_2$-norm across 5 public datasets.

==> REPLY.tex <==
Dear Chairs,
todo list:
1. rewrite the ethical consideration 
2. add [A]-[E] to related work
3. check reviewers' comments and make a table: (what they want, what we did/what content we add, where we add the new content)
4. complete ASR against 3 SOTA defense in appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Thank you very much.  

We've attached two PDF files: an 18-page final version and supplementary materials. 
The only difference in this version, compared to the previous uploaded version in the system, is the inclusion of [D]'s experimental results. 

Please note that a direct comparison between [D] (a clean-label attack) and LADDER was not feasible; instead, we converted [D] to a dirty-label variant to make the comparison.  
Obtaining all the experimental results took us roughly 40 hours.  

Tables II-IV show that LADDER achieves 13.6$\times$ better stealthiness (measured by $l_2$ norm), 1.78$\times$ better robustness and similar (only 0.16\% lower) attack effectiveness, as compared to [D].

In Tables XI-XIII, LADDER outperforms [D] by an average of 8.69\% in ASR, against SOTA defenses. 

The above results substantiate our previous claims in A11: 
> Since DUBA and [D] do not simultaneously address both stealthiness and robustness, their performance is lower than that of FIBA and our method. [DO NOT DELETE the symbols '> ']
[D]'s performance is worse than DUBA, FIBA and ours, w.r.t. three objectives and against SOTA defenses.

If any explanation or clarification is 
needed, we would be happy to provide details; if needed, we can also share the source code of the experiments. 

[D] "Narcissus: A practical clean-label backdoor attack with limited information," in ACM CCS, 2023.

########################################################################
- Comparison of SOTA. 
[A] uses a similar work from 2023 as a baseline and extends it to a dynamic variant that meets the dynamicity requirement. 
Notably, both [A] and NBA require limited knowledge to launch attacks: NBA operates as a static attack (triggered with a fixed position), whereas [A] requires a dynamic trigger design.

[B] incorporates four trigger designs in its framework but does not compare its results with other existing methods.

[C] compares its results with one classic attack and other related data-free attacks published before 2021.

[D] compares against related clean-label attacks and two classic (dirty-label) attacks, adapting these classic attacks to clean-label mode (before 2021).

[E] compares related patch-based attacks (before 2022).

Each of [A], [C], [D], and [E] selects related or similar attacks for comparison. Following the same philosophy/approach and comparison scale, we chose recent and related works such as FIBA and DUBA for our comparisons, as they address three specific objectives. 
As shown in Tables II, III, and IV, our method show advantages on all three objectives. 
Since DUBA and [D] do not simultaneously address both stealthiness and robustness, their performance is lower than that of FIBA and our method.

We acknowledge that various experimental setups could be tested, but the conclusions would remain unaffected. 
Furthermore, [D]'s experiments could not be completed within 12 HOURS; we began running them as soon as we saw the recent comments.

Finally, we emphasize that including every SOTA attack in our comparison is impractical, and indeed, no prior work (e.g., [A], [B], [C], [D], [E]) has done so. 
If the shepherd wishes for additional experiments, the shepherd should provide us more adequate time (rather than one day before 10/30) but also more interactions throughout the revision process. 

- Ethical considerations. 
[B], [C], [D] and [E] do not include any ethical statements, while only [A] briefly addresses ethical concerns related to personal or sensitive data, incorporating some protection mechanisms, such as encryption. 
In contrast, we exclusively use public datasets that do not contain any personal data, and thus we do not perceive any data-related risk. 
There is no foreseeable infringement on data privacy regulations. 
Given this context, data protection mechanisms like encryption are unnecessary, as our approach inherently avoids data privacy risks.
Furthermore, none of these works considers the potential misuse of their attacks. 
We address potential misuse by proposing a defense mechanism, detailed in the supplementary materials. 
If the shepherd has additional concerns or perceives any remaining risks, the shepherd should provide explicit guidance on which mechanisms or steps to incorporate to address these specific concerns.

[A] "FlowMur: A Stealthy and Practical Audio Backdoor Attack with Limited Knowledge," in IEEE S\&P, 2024.
[A]’s ethical consideration statements: 
[All human-related studies and experiments conducted in this paper have been approved by the Institutional Review Board of our institutes. Personal information, such as native language, age and region, was not recorded, except for the participants’ answers in the human study and their gender. Sensitive data, including gender, were encrypted and protected with access control.]
[B] "Sneaky Spikes: Uncovering Stealthy Backdoor Attacks in Spiking Neural Networks with Neuromorphic Data," in NDSS, 2024.
[C] "A data-free backdoor injection approach in neural networks," in USENIX Security, 2023.
[D] "Narcissus: A practical clean-label backdoor attack with limited information," in ACM CCS, 2023.
[E] "BadMerging: Backdoor Attacks Against Model Merging", in ACM CCS, 2024. 








Dear Shepherd, 

Thanks for the comments. 

1. Additional work

We confirm that our method achieves optimal performance w.r.t. three objectives as compared to the approach in 2024. 
We also include DUBA [24] in Table II, III and IV (please see the attached file). 
The current results in the tables demonstrate that our design achieves a higher average ASR ($>0.21\%$), with 1.33$\times$ stealthiness (measured by $l_2$ norm) and 1.78$\times$ robustness. 

During the revision, we've reviewed some SOTA backdoor attacks from security venues, for instance: 
[A] "FlowMur: A Stealthy and Practical Audio Backdoor Attack with Limited Knowledge," in IEEE S\&P, 2024.
[B] "Sneaky Spikes: Uncovering Stealthy Backdoor Attacks in Spiking Neural Networks with Neuromorphic Data," in NDSS, 2024.
[C] "A data-free backdoor injection approach in neural networks," in USENIX Security, 2023.
[D] "Narcissus: A practical clean-label backdoor attack with limited information," in ACM CCS, 2023.
[E] "BadMerging: Backdoor Attacks Against Model Merging", in ACM CCS, 2024. 



[A] focuses on speech recognition tasks instead of computer vision.
[B] considers Spiking Neural Networks (in spatial domain), which is different from CNNs.
[C] conducts backdoor attack without using original data/set. Instead, we target to data, designing the trigger to poison data. 
[D] only optimizes triggers in the spatial domain rather than dual domains.



To present a fair comparison, we only selected DUBA - the most recent and relevant work (with similar effect) - conducting a stealthy attack in dual domains and in black-box settings.  


2. Ethics

We provide further clarification on ethical considerations.

The libraries and data utilized in this paper are open-source, indicating that they possibly have undergone the community's review and are auditable. 
This transparency reduces the likelihood of hidden bugs and enhances the reliability of our experiments, particularly in the implementation of our backdoor approach and the corresponding potential defense. 
The datasets used are publicly available and have been extensively studied in existing literature. 
Since these are public datasets, their collection and processing do not involve any personal data, eliminating concerns related to privacy risks or data breaches. 
Our experiments also do not extend to real-world applications or human subjects. 
Moreover, we used these datasets solely within a secure and controlled virtual environment, without using them for any other purpose. 
The above confirms that this work does not yield any infringement on privacy regulations. 
We acknowledge, however, that there might be a risk of malicious use of our proposed backdoor attack. 
To address this, we propose an adaptive defense in ~\Cref{sec:possible_data_defense}.

%We here present more clarification for the ethical statement. 
%The libraries and data we used in this paper are open-source, indicating that they are reviewed and auditable by the community - reducing some hidden bugs and enhancing reliability in our experiments, in particular in the implementations of our backdoor and the corresponding potential defense.  
%The data used in this paper are from public datasets and well-studied in existing literature. Since the data are public, their collection and processing do not involve any personal data and thus do not incur issues like personal privacy risks and data breaches; our tests do not involve real-world applications and human. 
%Furthermore, we only used these tested data in a concealed and virtual environment rather than exposing them for other purposes.  
%The above confirms that this work does not yield any infringement on privacy regulations. 
%It is possible that malicious readers may misuse our designed backdoor attack. 
%To mitigate this risk, we propose an adaptive defense in~\Cref{sec:possible_data_defense}. 


%[Real-world risk]
%All backdoor algorithms were executed in a concealed and virtual environment, which brings no impact on any real-world applications. 
%This work will inspire the development of advanced technologies for more effective detection of invisible and robust triggers.
%It is crucial to note that this work could lead to backdoor techniques with potential safety risks, possibly enabling the development of more covertly malicious deep learning models.
%To recognize and mitigate the misuse of our backdoor attack, we propose an adaptive defense in~\Cref{sec:possible_data_defense}.
%[Privacy]
%Throughout the implementation and testing of LADDER, all comparative attacks, defenses, model architectures, and datasets were properly cited, publicly accessible, for academic use. 
%The datasets used in this work are widely recognized and studied in existing literature, with no risk of violating user privacy or data leakage, ensuring compliance with data privacy regulations such as GDPR. 
%To evaluate trigger stealthiness, we utilized mathematical models (metrics) to simulate human visual inspection thereby avoiding the need to involve real human subjects. 

% In summary, utilizes publicly available open-source libraries and publicly accessible resources including existing backdoor models, algorithms and datasets, does not collect or harm personal data, and ensures full compliance with privacy regulations.NDSS



We will upload the updated version in HotCRP.


==> abstract-bup.tex <==
\begin{abstract}

%Backdoor attacks inject trojans into deep neural networks by planting a \emph{trigger} into the training set during training, causing misclassification of poisoned images with an attacker-desired label during inference.
%In computer vision, most backdoor attacks either insert triggers in the spatial domain of an image where semantic information is comprehensible to humans, or manually manipulate patterns in the frequency domain. 
%However, both mechanisms in pixel and frequency domains introduce anomaly frequency artifacts between clean and poisoned data as well as taking risks of being removed by image processing operations such as compression and smoothing. 
%Consequently, a backdoor attack that simultaneously achieves dual-space stealthiness and robustness is in urgent demand.
%Aggregating and solving such multiple attack goals in \emph{single}-objective optimization problem is challenging.
%Current attacks aggregate objectives with Lagrange multipliers and optimize triggers with gradient descent, which is not only impractical in real-world scenarios where gradient information is inaccessible to attackers, but introduces excessive coefficients.
%Those coefficients are sensitive across datasets,  models and optimization problems, and result in unsatisfied attack performance when improperly configured.
%Moreover, we find the inherent conflict between the objectives of attack effectiveness and trigger stealthiness in backdoor attacks, and demonstrate that inaccurate Lagrange coefficients severely undermine the attack effectiveness due to the sensitivity and irreconcilable conflict among objectives.

%too long
%Here is the example: 
Backdoor attacks in deep neural networks misclassify images by inserting hidden \emph{triggers} during training. 
Current methods manipulate image's semantic or frequency patterns but risk removal by image processing operations due to anomaly frequency artifacts. 
%Hence, an urgent need for a backdoor attack that ensures both stealthiness and robustness. 
%Multiple attack goals present a challenge when consolidated into a single objective optimization problem. 
Furthermore, existing attacks proposed by using gradient descent and Lagrange multipliers are impractical and introduce excessive, sensitive coefficients resulting in poor attack performance when misconfigured. 
%The inherent conflict between attack effectiveness and trigger stealthiness critically hampers attack performance due to sensitivity and conflict among objectives.
%
We propose \textbf{e}volutionary \textbf{m}ulti-\textbf{o}bjective black-box \textbf{b}ackdoor \textbf{a}ttack in \textbf{f}requency domain (\textbf{EMOBAF}) that represents the first instance of considering dual-space stealthiness and robustness in multi-objective manner by customizing triggers in frequency domain.
%Intuitively, one may customize triggers by minimally perturbing low-frequency components of spectrum due to the inherent stealthiness and robustness achieved in this region. [explain these details in the main body]
%However, finding an optimal perturbation is non-trivial due to the intrinsic conflict among objectives such as attack effectiveness and stealthiness. [explain these details in the main body]
%Therefore, 
%EMOBAF leverages a multi-objective evolutionary algorithm on our proposed backdoor attack paradigm which maintains a set of trade-off triggers among objectives and heuristically variates them without relying on gradients until the backdoor attack achieves optimum. 
Thanks to evolutionary algorithm, EMOBAF can customize triggers stealthy in dual-space and robust to image preprocessing without gradient information in black-box setting. 
{\color{red}Extensive experiments comprehensively prove the attack effectiveness, attack robustness, inherent stealthiness in both spatial and frequency space as well as making it resilient against frequency inspection under the most practical scenarios. [revise this a bit to show some specific data/number here, e.g., in what performance under what datasets, what datasets are used? how much advantage we have???a concrete level of summary number???] } 

%just summarize what are the current issues? and then what we have proposed, what our proposal can do/achieve, and how the general experimental results look like = > then you get the abstract. 






%Backdoor attacks in computer vision inject Trojans into Deep Neural Networks during training, causing misclassification of poisoned images with an attacker-desired label during inference.
%Classic backdoor attacks achieve high attack effectiveness while preserving the model functionality on benign data by aggregating with Lagrange multiplier.
%Recently, other attack goals such as trigger stealthiness and robustness are considered. 
%These goals can be aggregated into classic backdoor attack with extra Lagrange coefficient.
%However, such an extension not only causes a growing number of parameters but leads to an unsatisfied attack performance when the objectives are sensitive to coefficients.
%%Meanwhile, this work for the first time reports that trigger effectiveness and stealthiness are mutually conflicting objectives, and hereby argue that formulating backdoor attack with Lagrange multiplier prevent objectives from achieving optimal simultaneously.
%Meanwhile, this study is the first to highlight the inherent conflict between trigger effectiveness and stealthiness in backdoor attacks. We demonstrate that introducing Lagrange multipliers for conflicting objectives makes it hard to seek optimal.
%Moreover, existing stealthy backdoor attacks either insert triggers in spatial domain where pattern is visible to human eyes; or handcraft fixed patterns in frequency domain, which not only introduces noticeable frequency disparities between clean and poisoned data but also take risks of being removed by image preprocessing.

%Addressing the above drawbacks we propose \textbf{e}volutionary \textbf{m}ulti-\textbf{o}bjective robust and stealthiness \textbf{b}lack-box backdoor \textbf{a}ttack in \textbf{f}requency domain (\textbf{EMOBAF}). 
%which represent the first instance of considering attack effectiveness, stealthiness and robustness in multi-objective manner without introducing any aggregation coefficients.
%Furthermore, our EMOBAF is the first method to customize triggers by consider stealthiness in \emph{dual-space}, which avoids both the visual and frequency residual anomaly at the same time.
%Specifically, EMOBAF customizes trigger by perturbing low-frequency components in spectrum due to the inherit stealthiness and robustness achieved in this region.
%Then, we leverage multi-objective evolutionary algorithm to our novel backdoor attack paradigm, which divides the original backdoor tasks into sub-problems with various trade-offs among objectives. 
%Finally, frequency triggers (includes the magnitude of perturbations and locations to pose them on) for each sub-problem is repeatedly updated until the backdoor attack achieves optimal.
%Extensive experiments on x real-world datasets against x comparison attacks, x image processing methdos and x defenses comprehensively proved the attack effectiveness, attack robustness, inherent stealthiness in both spatial and frequency space as well as making it resilient against frequency inspection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%Deep neural networks (DNNs) have demonstrated a huge success in computer vision, such as EG1 and EG2. However, yet is still vulnerable to backdoor attacks. 
%Deep neural networks (DNNs) is heavily threatened by backdoor attack.
%In computer vision, backdoor attack injects a Trojan into DNNs with maliciously conducted images during training so that, upon inference, poisoned images are misclassified with an attacker-desired label. 
%Most backdoor attacks inject trigger into images in spatial domain where semantic information is comprehensible to humans. 
%Consequently, triggers can be easily detected by visual inspection.
%Recent works plant fixed patterns in frequency domain, which reflects indistinguishable pixel-wise perturbations.
%However, frequency triggers introduces anomaly frequency disparities between clean and poisoned data as well as taking risks of being removed by image processing operations, such as compression and smoothing.
%Moreover, we found that attack effectiveness and stealthiness are mutually conflicting objectives, the commonly used aggregation-oriented backdoor paradigm relying on Lagrange multiplier can hardly achieve satisfied trade-offs. 
%%In short, existing backdoor attacks never achieve the threefold-stealthiness, i.e., stealthiness in spatial space, frequency space and latent representation space.

%This work represents the first instance to considers attack effectiveness, dual-space stealthiness and robustness simultaneously via a novel multi-objective backdoor attack paradigm, which ingeniously customizes trigger by dataset in frequency domain.
%Besides, our backdoor paradigm does not rely on gradient or parameter from model, hereby adapts well in black-box scenario, the most challenging backdoor setup.
%Meanwhile, we introduce a heterogeneous surrogate model for trigger generation process and empirically prove the transferable of attack effectiveness between surrogate and real model, which makes our attack more practical on black-box setting.
%Eventually, we formulate an \textbf{e}volutionary \textbf{m}ulti-\textbf{o}bjective robust and stealthiness \textbf{b}lack-box backdoor \textbf{a}ttack in \textbf{f}requency domain (\textbf{EMOBAF}). 
%Specifically, EMOBAF customizes trigger by perturbing low-frequency components in frequency spectrum due to {\color{red}our discovery the inherit stealthiness and robustness is achieved in this region.} 
%Then, we leverage multi-objective evolutionary algorithm to our novel backdoor attack paradigm, which divides the original backdoor tasks into sub-problems with various trade-offs among objectives. 
%Finally, frequency triggers (includes the magnitude of perturbations and locations to pose them on) for each sub-problem is repeatedly updated until the backdoor attack achieves optimal.
%Extensive experiments on x real-world datasets against x comparison attacks, x image processing methdos and x defenses comprehensively proved the attack effectiveness, attack robustness, inherent stealthiness in both spatial and frequency space as well as making it resilient against frequency inspection.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{abstract}

==> archived.tex <==
%Backdoor attacks in computer vision involve injecting Trojans into Deep Neural Networks (DNNs) during training, causing misclassification of poisoned images with an attacker-desired label during inference.
%Most backdoor attacks inject trigger into images in spatial domain where semantic information is comprehensible to humans. 
%Consequently, triggers can be easily detected by visual inspection.
%Recent works embed handcrafted patterns in frequency domain, resulting in a visually indistinguishable pixel-wise perturbations yet introduce noticeable frequency disparities between clean and poisoned data
%Meanwhile, those handcrafted trigger patterns take risks of being removed by image preprocessing.
%Therefore, A mitigation capable of producing triggers by considering multiple attack goals such as effectiveness, robustness and stealthiness is in urgent demand.
%A few works formulate backdoor attack concerning multiple objectives, which leverage Lagrange multiplier to construct their attack as a single-objective problem.

==> intro-bup.tex <==
\section{Introduction}
\label{sec:intro}

With the development of machine learning (ML) \citep{bishop2013pattern}, deep neural networks (DNNs) \citep{Goodfellow-et-al-2016} have become effective ML implementations for image classification. 
They are proved to be vulnerable to backdoor attacks \citep{fiba,badnets,wanet}, which mislead a victim model to make attacker-desired predictions on poisoned images during inference while maintaining normal behaviors on clean images.
These attacks pose severe risks to a wide range of practical vision systems, such as tumor diagnosis \citep{esteva2017dermatologist} and autopilot \citep{autodriving}. 
%Henceforth, the advancement of a powerful backdoor attack is an urgent need to verify the security of DNN-based systems and orient the development of advanced backdoor defenses.

Conventional pixel-based backdoor attacks achieve success by injecting triggers into spatial domain \citep{badnets}. 
Since spatial domain contains abundant semantic information understandable to humans, inserting triggers into pixels severely harms semantics in human recognition, making poisoned images easily detectable by visual inspection.
% As a consequence, poisoned images can be easily detected by visual inspection. 
Recent research carries on backdoor attacks by injecting triggers into frequency domain \citep{ft,fiba,LFAP}. 
% FTrojan \citep{ft} is one of the most typical methods in this category. 
Inspired by patch-based backdoor attacks, FTrojan \citep{ft} manipulates the mid- and high-frequency spectrum of images by inserting predefined perturbations to fixed frequency bands. 
Manually crafting frequency components, especially in high-frequency regions, harms the trigger robustness since most image processing operations such as low-pass filters and image compression such as JPEG clip the high-frequency components (see \Cref{fig:smoothing_disparity}). 
Moreover, current spatial and frequency triggers introduce distinguishable artifacts in frequency and/or spatial domain (see \Cref{fig:freq_disparity_map}), which bear a high risk of existing attacks being detected.

Studies \citep{Wang2023RobustBA,color} conclude that an ideal backdoor attack should fulfill \emph{stealthiness}, \emph{robustness}, \emph{effectiveness} and \emph{functionality preservation}.
Stealthiness naively concerns a trigger in the poisoned image to be stealthy to human visual perception.
Robustness is evidenced by its ability to withstand image processing and resist countermeasures against backdoor defenses.
Effectiveness requires that backdoor to be successfully injected into the victim model and capable of being activated with a high attack success rate upon inference, while functionality preservation requires inference accuracy remain unaffected on benign data.

This work inherits and extends stealthiness in two-folded, referred to as \emph{dual-space stealthiness}: (1) spatial stealthiness, which guarantees the injection of trigger into the image does not destroy cognitive semantics or introduce visual anomaly, and (2) frequency domain stealthiness, which requires to avoid the disparities of frequency spectrum between clean images and their poisoned counterparts.
On top of that, the backdoor injection should keep the functionality of victim model on benign tasks as much as possible. 
Despite the stealthiness achieved by \citep{Wang2023RobustBA} at pixel level, we shed lights on stealthiness in frequency domain as well as guaranteeing all the attack goals mentioned above.

\begin{figure}[!bpt]
    \centering
    \scalebox{0.46}{\includegraphics{images/main_workflow_chatV4.pdf}}
    \caption{The workflow of EMOBAF. 
    Step \ding{172}\textasciitilde\ding{174}: trigger injection;
    Step \ding{175}\textasciitilde\ding{177}: main loop for trigger optimization;
    Step \ding{178}\textasciitilde\ding{179}: poison dataset with trigger and release it to public;
    Step \ding{180}: the backdoor is injected when users download the poisoned data to train/tune their own model.
    The trigger optimization, evaluation, injection are controlled by an attacker, whereas the malicious training and inference stage (marked in grey) are unseen to the attacker.
    }
    \label{fig:EMOBAF_workflow_chat}
\end{figure}

It has been well claimed that low-frequency components of natural images contain semantic information understandable to humans, whereas high-frequency ones stand for details and noise \citep{watermark}. 
Based on this, works \citep{watermark,LFAP} state two benefits of inserting triggers in low-frequency domain: 
(1) abundant information contained in low-frequency domain can provide a high perceptual capacity of accommodating trigger patterns without perceptual degradation, which improves the degree of trigger stealthiness; 
and (2) low-frequency components can bear a better resilience in image compression and are less prune to be removed by image filtering than component, which guarantees a better attack robustness. 

The aforementioned insights underscore the urgent need for a backdoor attack that can generate triggers in the low-frequency region while ensuring dual-space trigger effectiveness and stealthiness without necessitating knowledge of the victim model structure as well as being robust against preprocessing operations.
However, searching an optimal trigger that meets multiple objectives in an advanced backdoor attack is non-trivial due to the following challenges:
\textbf{(C1)} due to the practical but strict assumption in black-box setting where the target model is inaccessible to attackers, it is not possible to acquire gradient information or predict trigger performance on the victim model and is therefore hard to find optimal trigger with gradient descent;
\textbf{(C2)} the objectives of attack effectiveness and trigger stealthiness are mutually conflicting, which prevent objectives from achieving best simultaneously.
Meanwhile, leveraging Lagrange multiplier on multiple attack objectives, as did by the mainstream \citep{ImperceptibleBD,defeat}, introducing excessive coefficients.
Due to the sensitivity of coefficients to the defined optimization problem as well as various datasets and model architectures, 
it is difficult to seek optimal triggers whose attack effectiveness and trigger stealthiness are all desired by the attackers;
and \textbf{(C3)} 
improperly handcrafted fixed triggers in spectrum (with fixed magnitude of perturbations and locations) lead to improper signal in spectrum or limited attack effectiveness. 
For example, a trigger with large perturbations such as \citep{ft, fiba} disrupts invisibility or even destroy original semantics of images, whereas a trigger with small perturbation prevents model from learning the trigger pattern, resulting in low attack effectiveness.

This paper addresses the above challenges $C1\sim C3$ with EMOBAF, a novel black-box backdoor attack which leverages multi-objective evolutionary algorithm (MOEA), a gradient free hyper-heuristics, to effectively search triggers in frequency domain (see \Cref{fig:EMOBAF_workflow_chat} for the overall workflow). 
Thanks to MOEA, our EMOBAF solves the objectives of atack effectiveness and dual-space stealthiness simultaneously without aggregating objectives by Lagrange multiplier, hereby avoid assigning budget on tuning sensitive coefficients and obtains better trigger (see \Cref{fig:paretoFront}).
Meanwhile, EMOBAF maintains a population of triggers which adaptively approximate different trade-offs among objectives against each other, so that all objectives are optimized at the same time and Lagrange coefficients are not required when obtaining triggers (mitigation for \textbf{C2}). 
Specifically, EMOBAF first converts an image into spectrum with discrete cosine transform (DCT\footnote{Without loss of generality, we choose type-II DCT and its inversion for this work due to their widespread usage in the literature.}). 
Then, a trigger is randomly generated and heuristically optimized with EA guided by the trajectory of previous iterations in order to minimally perturbing the magnitude and location of perturbations while maintains a satisfied attack effectiveness (mitigation for \textbf{C3}). 
Along the trigger optimization iteration, we integrate a preference based selection into EMOBAF, so that the triggers are obtained along the sub-region where all objectives are preferred by attackers, which enables EMOBAF to efficiently search triggers in an immense search space (mitigation for \textbf{C2}).
Finally, we apply inverse DCT (IDCT) on the poisoned frequency spectrum to obtain the poisoned images. 
To evaluate triggers during EMOBAF iteration, we construct a surrogate model tuned on a subset of training data due to the model inaccessibility in black-box setup.
Since the optimization direction guided by gradient information of victim model is also unknown, we drive triggers toward optimal with variation (crossover and mutation) and selection pressure which are inspired by the mating and survival of natural evolution (mitigation for \textbf{C1}).
We empirically confirm that the trigger performance is independent to model structures, and this way a heterogeneous surrogate model is capable of approximate the victim model in an acceptable accuracy and stealthiness. 

The \textbf{main contributions} of this paper can be summarized as follows:

\noindent{\(\bullet\)}
We provide a new perspective of designing trigger in the frequency domain, which guarantees the stealthiness in both spatial and frequency domain, the attack robustness against image preprocessing as well as the attack effectiveness.

\noindent{\(\bullet\)}We find the intrinsic conflict among attack objectives such as trigger stealthiness and attack effectiveness, which intriguing the sensitivity of widely used Lagrange multiplier with SGD from executing backdoor attack across datasets and model structures. 

\noindent{\(\bullet\)} Building on this, we formulate backdoor attack as a novel multi-objective paradigm where objectives are optimized simultaneously without relying on gradients. 
As a result, our approach proves effective in black-box settings, significantly enhancing its practicality.


\noindent{\(\bullet\)} Extensive experiments confirm that EMOBAF achieves state-of-the-art attack effectiveness, robustness against various spatial, frequency, and image transformation defenses.



%\noindent{\(\bullet\)We search trigger in frequency domain, and we focus on attack in low-frequency domain.}\\
%\noindent{\(\bullet\)With the help of frequency-domain trigger, we guarantee a dual-space stealthiness as well as the attack robustness against popular defensive such as STRIP, neuron-cleansing and etc.}\\
%\noindent{\(\bullet\)We formulate attack in an multi-objective optimization problem, and solve the problem with multi-objective evolutionary algorithm.}\\
%\noindent{\(\bullet\)thanks to our multi-objective backdoor attack formulation, parameters of Lagrange coefficient is not required, which not only enables our attack to be parameter free but also makes it scalable to more objectives.}\\
%\noindent{\(\bullet\) Extensive experiments empirically confirm that our EMOBAF provides cutting-edge backdoor effectiveness, robustness and stealthiness against current spatial and frequency attacks as well as achieves robustness against commonly recognized defenses.}



